L-Sort: On-chip Spike Sorting with Efficient Median-of-Median Detection and Localization-based Clustering

Spike sorting is a critical process for decoding large-scale neural activity from extracellular recordings. The advancement of neural probes facilitates the recording of a high number of neurons with an increase in channel counts, arising a higher data volume and challenging the current on-chip spike sorters. This paper introduces L-Sort, a novel on-chip spike sorting solution featuring median-of-median spike detection and localization-based clustering. By combining the median-of-median approximation and the proposed incremental median calculation scheme, our detection module achieves a reduction in memory consumption. Moreover, the localization-based clustering utilizes geometric features instead of morphological features, thus eliminating the memory-consuming buffer for containing the spike waveform during feature extraction. Evaluation using Neuropixels datasets demonstrates that L-Sort achieves competitive sorting accuracy with reduced hardware resource consumption. Implementations on FPGA and ASIC (180 nm technology) demonstrate significant improvements in area and power efficiency compared to state-of-the-art designs while maintaining comparable accuracy. If normalized to 22 nm technology, our design can achieve roughly $\times 10$ area and power efficiency with similar accuracy, compared with the state-of-the-art design evaluated with the same dataset. Therefore, L-Sort is a promising solution for real-time, high-channel-count neural processing in implantable devices.

==> obsolete/sota_obsolete.tex <==
\begingroup
\renewcommand{\arraystretch}{1.2}
\begin{table*}[t]
\centering
\caption{State-of-the-art On-chip Spike Sorting}
\label{table:sota}
%\resizebox{\linewidth}{!}{%
\begin{threeparttable}
\setlength\tabcolsep{5pt}
\begin{tabular}{|cc|c|c|c|c|c|c|c|}
\hline
\multicolumn{2}{|c|}{Work}                                                                                      & \begin{tabular}[c]{@{}c@{}}ESSCIRC'2018\\ \cite{li2018esscirc}\end{tabular} & \begin{tabular}[c]{@{}c@{}}TVLSI'2019\\ \cite{tuan2019tvlsi}\end{tabular} & \begin{tabular}[c]{@{}c@{}}TBCAS'2021\\ \cite{han2021tbcas}\end{tabular} & \begin{tabular}[c]{@{}c@{}}TVLSI'2022\\ \cite{fereshteh2022tvlsi}\end{tabular} & \begin{tabular}[c]{@{}c@{}}TBCAS'2022\\ \cite{zeinolabedin2022tbcas}\end{tabular} & \begin{tabular}[c]{@{}c@{}}JSSC'2023\\ \cite{jssc_2023}\end{tabular} & \textbf{This work}    \\ \hline
\multicolumn{1}{|c|}{\multirow{3}{*}{Algorithm}} & \begin{tabular}[c]{@{}c@{}}Spike\\ Detection\end{tabular}    & \begin{tabular}[c]{@{}c@{}}Absolute\\ thresholding\end{tabular}             & ICD                                                                       & \begin{tabular}[c]{@{}c@{}}Absolute\\ thresholding\end{tabular}          & \begin{tabular}[c]{@{}c@{}}Absolute\\ thresholding\end{tabular}                & NEO                                                                               & NEO                                                                  & \textbf{Median}       \\ \cline{2-9} 
\multicolumn{1}{|c|}{}                           & \begin{tabular}[c]{@{}c@{}}Feature\\ Extraction\end{tabular} & \begin{tabular}[c]{@{}c@{}}Max-min\\ detection\end{tabular}                 & \begin{tabular}[c]{@{}c@{}}Integer\\ coefficient\end{tabular}             & FSDE                                                                     & Not applied                                                                    & \begin{tabular}[c]{@{}c@{}}Adaptive\\ filter\end{tabular}                         & Peak-FSDE                                                            & \textbf{Location}     \\ \cline{2-9} 
\multicolumn{1}{|c|}{}                           & Clustering                                                   & \begin{tabular}[c]{@{}c@{}}1.5D Bayesian\\ boundary\end{tabular}            & \begin{tabular}[c]{@{}c@{}}Modified\\ K-means\end{tabular}                & \begin{tabular}[c]{@{}c@{}}Perturbed\\ K-means\end{tabular}              & \begin{tabular}[c]{@{}c@{}}CC-based\\ clustering\end{tabular}                  & Configurable                                                                      & Geo-OSort                                                            & \textbf{OSort}        \\ \hline
\multicolumn{2}{|c|}{Number of channels}                                                                        & 96                                                                          & 128                                                                       & 4                                                                        & 64                                                                             & 16                                                                                & 384                                                                  & \textbf{384}          \\ \hline
\multicolumn{2}{|c|}{Dataset}                                                                                   & -                                                                           & Quiroga                                                                   & Quiroga                                                                  & Quiroga                                                                        & Quiroga                                                                           & Neuropixel                                                           & \textbf{Neuropixel}   \\ \hline
\multicolumn{2}{|c|}{Accuracy}                                                                                  & -                                                                           & 72\%                                                                      & 93.2\%                                                                   & 85\%                                                                           & 94.1\%                                                                            & 97.7\%                                                               & \textbf{98.3\%}       \\ \hline
\multicolumn{2}{|c|}{Technology}                                                                                & 180nm                                                                       & 65nm                                                                      & 180nm                                                                    & 180nm                                                                          & 22nm                                                                              & 22nm                                                                 & \textbf{180nm}        \\ \hline
\multicolumn{2}{|c|}{Core Voltage}                                                                              & 0.32V                                                                       & 0.54V                                                                     & 1.5V                                                                     & 1.8V                                                                           & 0.5V-0.8V                                                                         & 0.59V                                                                & \textbf{1.8V}         \\ \hline
\multicolumn{2}{|c|}{\begin{tabular}[c]{@{}c@{}}Number of Bits of\\ Input Data\end{tabular}}                    & 8-bit                                                                       & 9-bit                                                                     & Analog input                                                             & 8-bit                                                                          & 9-bit                                                                             & 12-bit                                                               & \textbf{12-bit}       \\ \hline
\multicolumn{2}{|c|}{\begin{tabular}[c]{@{}c@{}}Sampling Rate of\\ Input Data\end{tabular}}                     & 30kHz                                                                       & 25kHz                                                                     & 24kHz                                                                    & 25kHz                                                                          & 25kHz                                                                             & 30kHz                                                                & \textbf{30kHz}        \\ \hline
\multicolumn{2}{|c|}{Power per channel}                                                                         & 0.006$\mu$W                                                                 & 0.175$\mu$W                                                               & 4.68$\mu$W                                                               & 1.74$\mu$W                                                                     & 2.79$\mu$W                                                                        & 1.78$\mu$W                                                           & \textbf{71.03$\mu$W} \\ \hline
\multicolumn{2}{|c|}{Area per channel}                                                                          & 0.019mm$^2$                                                                 & 0.003mm$^2$                                                               & 1.023mm$^2$                                                              & 0.047mm$^2$                                                                    & 0.014mm$^2$                                                                       & 0.0013mm$^2$                                                         & \textbf{0.0033mm$^2$} \\ \hline
\multicolumn{2}{|c|}{Normalized power per channel\dag}                                                          & 0.190$\mu$W                                                                 & 12.416$\mu$W                                                              & 6.74$\mu$W                                                               & 1.74$\mu$W                                                                     & 779.10$\mu$W                                                                      & 566.74$\mu$W                                                         & \textbf{71.03$\mu$W} \\ \hline
\multicolumn{2}{|c|}{Normalized area per channel\dag}                                                           & 0.019mm$^2$                                                                 & 0.036mm$^2$                                                               & 1.023mm$^2$                                                              & 0.047mm$^2$                                                                    & 1.162mm$^2$                                                                       & 0.1079mm$^2$                                                         & \textbf{0.0033mm$^2$} \\ \hline
\end{tabular}
\begin{tablenotes}
    \item[\dag] normalized to 180nm with 1.8V voltage supply using scaling factors from~\cite{scale}.
\end{tablenotes}
\end{threeparttable}
%}
\end{table*}
\endgroup
